Automated and manual testing as part of the research software development process of RCE

Research software is often developed by individual researchers or small teams in parallel to their research work. The more people and research projects rely on the software in question, the more important it is that software updates implement new features correctly and do not introduce regressions. Thus, developers of research software must balance their limited resources between implementing new features and thoroughly testing any code changes. We present the processes we use for developing the distributed integration framework RCE at DLR. These processes aim to strike a balance between automation and manual testing, reducing the testing overhead while addressing issues as early as possible. We furthermore briefly describe how these testing processes integrate with the surrounding processes for development and releasing.

==> images/artifacts.tex <==
\newsavebox{\lockbox}
\savebox\lockbox{
\begin{tikzpicture}[thick,scale=.4]
  \draw (0,0) -| (1,1) -| cycle;
  \draw (0,.5) -- (1,.5);
  \draw (0,.6) -- (1,.6);
  \draw (0,.7) -- (1,.7);
  \draw (.5,.1) -- (.5,.4);

  \draw (.25,1) -- (.25,1.25) arc[start angle=180, end angle=0, radius=.25] -- (.75,1);
\end{tikzpicture}
}

\begin{tikzpicture}[xscale=2.5,yscale=1.2,thick]
  \node (codebase) at (1,0) {Codebase};

  \node[align=center] (update-site) at (-1,-.75) {Update\\Site};

  \node[align=center] (zip-windows) at (0,-.75) {Zip File\\(Windows)};
  \node[align=center] (zip-windows-sign) at (0,-1.75) {\usebox{\lockbox}};

  \node[align=center] (zip-linux) at (1,-.75) {Zip File\\(Linux)};

  \node[align=center] (zip-linux-sign) at (1,-1.75) {\usebox{\lockbox}};
  \node[align=center] (deb) at (2,-.75) {.deb\\Package};
  \node[align=center] (rpm) at (3,-.75) {.rpm\\Package};

  \node[align=center] (apt) at (2,-1.75) {Debian\\Repository};

  \path[draw,->,rounded corners] (codebase) -| (update-site);
  \path[draw,->,rounded corners] (codebase) -| (zip-windows);
  \path[draw,->,rounded corners] (codebase) -- (zip-linux);
  \path[draw,->,rounded corners] (codebase) -| (deb);
  \path[draw,->,rounded corners] (codebase) -| (rpm);

  \path[draw,->,rounded corners] (zip-windows) -- (zip-windows-sign);

  \path[draw,->,rounded corners] (zip-linux) -- (zip-linux-sign);

  \path[draw,->,rounded corners] (deb) -- node[anchor=west] {\scalebox{.5}{\usebox{\lockbox}}} (apt);
\end{tikzpicture}


==> images/vph-infrastructure.tex <==
\newsavebox{\serverbox}
\savebox\serverbox{
\begin{tikzpicture}[thick]
	\node[draw,rounded corners=.1cm,minimum height=.075cm,minimum width=1.2cm,fill=white] at (0,0) {};
	\node[circle,minimum size=.1cm,fill=black,inner sep=0] at (-.4cm,0cm) {};
	
	\node[draw,rounded corners=.1cm,minimum height=.075cm,minimum width=1.2cm,fill=white] at (0,.35) {};
	\node[circle,minimum size=.1cm,fill=black,inner sep=0] at (-.4cm,.35) {};
	
	\node[draw,rounded corners=.1cm,minimum height=.075cm,minimum width=1.2cm,fill=white] at (0,.7) {};
	\node[circle,minimum size=.1cm,fill=black,inner sep=0] at (-.4cm,.7) {};
\end{tikzpicture}
}

\newsavebox{\desktopbox}
\savebox\desktopbox{
\begin{tikzpicture}[outer sep=0,inner sep=0]
	\draw[thick,rounded corners=.1cm,line width=.08cm,fill=white]
		(0,0) -- (.5,0) -- (.5,.7) -- (-.5,.7) -- (-.5,0) -- cycle;
		
	\draw[thick,rounded corners] (0,0) -- (0,-.2);
	\draw[thick,rounded corners] (-.3,-.18) -- (.3,-.18);
\end{tikzpicture}
}

\begin{tikzpicture}[thick,xscale=2,yscale=1.5]

\tikzset{system/.style = {inner sep=0}}
\tikzset{network/.style = {draw,rounded corners,fill=black!10,inner sep=.2cm}}
\tikzset{network gateway/.style = {shape=rectangle,draw,fill=black!10,minimum size=.5cm,thick}}
\tikzset{network connection/.style = {draw,rounded corners,stealth-stealth,thick}}

\node[system] (partner-3-1) at (1.5,1.5) {\usebox{\desktopbox}};
\node[system] (partner-3-2) at (1.5,0.5) {\usebox{\desktopbox}};

\begin{pgfonlayer}{background}
  \node[network,fit = (partner-3-1) (partner-3-2),label=right:{\rotatebox{-90}{Partner \textsc{III}}}] (partner-3-network) {};
\end{pgfonlayer}

\node[system] (partner-2-1) at (-2,1.5) {\usebox{\desktopbox}};
\node[system] (partner-2-2) at (-1,1.5) {\usebox{\desktopbox}};
\node[system] (partner-2-3) at (-1.5,0.5) {\usebox{\serverbox}};


\begin{pgfonlayer}{background}
  \node[network,fit = (partner-2-1) (partner-2-2) (partner-2-3),label=left:{\rotatebox{-90}{Partner \textsc{II}}}] (partner-2-network) {};
\end{pgfonlayer}

\node[system] (partner-1-1) at (-2,-1) {\usebox{\desktopbox}};
\node[system] (partner-1-2) at (-1,-1) {\usebox{\desktopbox}};
\node[system] (partner-1-3) at (0,-1) {\usebox{\serverbox}};
\node[system] (partner-1-4) at (1,-1) {\usebox{\serverbox}};
\node[system] (partner-1-5) at (2,-1) {\usebox{\desktopbox}};

\node[system] (partner-1-relay) at (0,0.5) {\usebox{\serverbox}};

\begin{pgfonlayer}{background}
  \node[network,fit = (partner-1-1) (partner-1-5),label=below:{Partner \textsc{I}},inner ysep=.3cm,yshift=.25cm] (partner-1-network) {};
  \draw[rounded corners,pattern=north east lines,pattern color=black!35] (partner-1-2.north |- partner-1-network.north) -| (partner-1-relay.west) |- ($(partner-1-relay.north) + (0,.2)$) -| (partner-1-relay.east) |- (partner-1-4.north |- partner-1-network.north) -- cycle;
  \node[network,fit = (partner-1-1) (partner-1-5),label=below:{Partner \textsc{I}},inner ysep=.3cm,yshift=.25cm] (partner-1-network) {};
\end{pgfonlayer}

\path[network connection] (partner-3-1) -| ($(partner-3-1) ! .5 ! (partner-1-relay)$) |- (partner-1-relay);
\path[network connection] (partner-3-2) -- (partner-1-relay);

\path[network connection] (partner-2-1) -| (partner-2-3);
\path[network connection] (partner-2-2) -| (partner-2-3);
\path[network connection] (partner-2-3) -- (partner-1-relay);

\path[network connection] (partner-1-1.north) |- ($(partner-1-3.north) + (0,.2cm)$) -- (partner-1-relay);
\path[network connection] (partner-1-2.north) |- ($(partner-1-3.north) + (0,.2cm)$) -- (partner-1-relay);
\path[network connection] (partner-1-3.north) -- (partner-1-relay);
\path[network connection] (partner-1-4.north) |- ($(partner-1-3.north) + (0,.2cm)$) -- (partner-1-relay);
\path[network connection] (partner-1-5.north) |- ($(partner-1-3.north) + (0,.2cm)$) -- (partner-1-relay);

\node[anchor=south,align=center] (dmz) at ($(partner-1-relay.north) + (0,.2)$) {Partner \textsc{I}\\DMZ};
\end{tikzpicture}

